Regular polytopes, sphere packings and Apollonian sections

In this paper, we explore the geometry and the arithmetic of a family of polytopal sphere packings induced by regular polytopes in any dimension. We prove that every integral polytope is crystallographic, and we show that there are 11 crystallographic regular polytopes in any dimension. After introducing the notion of Apollonian section, we determine which Platonic crystallographic packings emerge as cross-sections of the Apollonian arrangements of the regular 4-polytopes. Additionally, we compute the M\"obius spectrum of every regular polytope.

==> sections/conclusion.tex <==
%
%
%
%We conclude with the following conjecture on the numbers appearing in the two remarkable regular crystallographic sphere packings depicted in Figure \ref{fig:conj24}.
%\begin{conj} The set of bends of the hypercubic and 24-cell crystallographic packings
%	$\mathscr P_{\{4,3,3\}}(0,0,1,2)$ and $\mathscr P_{\{3,4,3\}}(0,0,1,2)$ is $\mathbb N$.
%\end{conj}
%
%
%\begin{figure}[H]
%	\centering
%	\begin{tabular}{cc}
%		\includegraphics[align=c,width=0.45\textwidth]{img/gaskets/433gasket0011v3}			&	\includegraphics[clip,trim=0 80 0 80,align=c,width=0.4\textwidth]{img/gaskets/343gasket0011}
%		%$\mathscr P_{\{4,3,3\}}(0,0,1,2)$&$\mathscr P_{\{3,4,3\}}(0,0,1,2)$
%	\end{tabular}	
%	\caption{(Left) The integral hypercubic crystallographic packing $\mathscr P_{\{4,3,3\}}(0,0,1,2)$. (Right) The integral 24-cell crystallographic packing $\mathscr P_{\{3,4,3\}}(0,0,1,2)$.}
%	\label{fig:conj24}
%\end{figure}



